Pruning Deep Convolutional Neural Network Using Conditional Mutual Information

Convolutional Neural Networks (CNNs) achieve high performance in image classification tasks but are challenging to deploy on resource-limited hardware due to their large model sizes. To address this issue, we leverage Mutual Information, a metric that provides valuable insights into how deep learning models retain and process information through measuring the shared information between input features or output labels and network layers. In this study, we propose a structured filter-pruning approach for CNNs that identifies and selectively retains the most informative features in each layer. Our approach successively evaluates each layer by ranking the importance of its feature maps based on Conditional Mutual Information (CMI) values, computed using a matrix-based Renyi {\alpha}-order entropy numerical method. We propose several formulations of CMI to capture correlation among features across different layers. We then develop various strategies to determine the cutoff point for CMI values to prune unimportant features. This approach allows parallel pruning in both forward and backward directions and significantly reduces model size while preserving accuracy. Tested on the VGG16 architecture with the CIFAR-10 dataset, the proposed method reduces the number of filters by more than a third, with only a 0.32% drop in test accuracy.

==> background.tex <==
\section{Background}

\subsection{Convolutional Neural Network}
 Convolutional Neural Network (CNN) is a specialized type of deep neural network primarily used for processing structured grid-like data such as images  \citep{younesi_2024_comprehensive}. CNN is particularly effective in image processing tasks such as image classification or object detection, because of its ability to automatically learn and extract \emph{hierarchical features} from the input data. Different CNN architectures have been introduced for image processing tasks, including LeNet \citep{lecun_1998_gradient}, AlexNet \citep{krizhevsky_2012_imagenet}, Visual Geometry Group (VGG) \citep{simonyan_2014_very}, Residual Network (ResNet) \citep{he_2016_deep} and MobileNet \citep{howard_2017_mobilenets}. \mv{Is this citation list in any particular order?} \noteblue{Tien edited citation list in ascending order by year}

A CNN architecture generally consists of an input layer, a stack of alternating convolutional and pooling layers, several fully connected layers, and an output layer at the end \citep{zhao_2024_review}. The top panel in Fig. \ref{fig:process_of_CNN} shows the VGG-16 architecture, which includes 13 convolutional layers and 3 fully connected layers. Each convolutional layer contains a set of filters. A convolution operation involves sliding a filter over the input image, multiplying the filter values by the pixel values at corresponding positions in the input image, and summing the results to obtain a feature map. By applying various filters to the input image, a set of feature maps is generated, as shown in Fig. \ref{fig:process_of_CNN}. When multiple convolutional layers are stacked, the later layers capture more representative features of the input image. We will use the VGG-16 architecture as the main example for implementation in this paper, but all the discussion and developed algorithms can be applied to any CNN structure.


\begin{figure}[h]
\begin{center}
\includegraphics[width=0.8\textwidth]{images/process_of_CNN.drawio.png}
\end{center}
\caption{Illustration of the process of a sample CNN model.}
\label{fig:process_of_CNN}
\end{figure}
%https://app.diagrams.net/#G1nNosWbkqZQE_GFxAzLEoY4yt5LG5-AKM#%7B%22pageId%22%3A%22Fo-Tg2ZRT6S6ixIx0M7V%22%7D




%\nguyen{We should discuss multivariate MI computation using Reyni entropy here.}

%\mv{This is TOO MUCH detail. Dilute the focus. May just refer to a reference for this section. Our method does NOT depend on Reyni, it is just a technique for computing the MI.}

%\nguyen{I will edit this section.}

%\notered{Chị Nguyên revise lại phần này}

\subsection{Multivariate mutual information using Rényi entropy} 

Our proposed CNN pruning method is based on computing the conditional mutual information between the features extracted in the same layer and in different layers of the CNN. Each feature is treated as a multivariate random variable in matrix form. The test data after being processed through the trained CNN provides samples or realizations of each random feature at each layer. Next, we discuss the method used for computing the mutual information (MI) and conditional mutual information (CMI) subsequently.

\textbf{Rényi Entropy and Mutual Information Computation:} 
To estimate MI between random variables, we rely on the Rényi's $\alpha$-order entropy $H_\alpha(X)$ ~\citep{renyi1965foundations}, defined as %Generally, entropy quantifies the uncertainty of random variables using a single scalar quantity. 
%For a continuous random variable $X$ with a probability density function (PDF) $p(x)$ defined on the set $X$, the $\alpha$-order Renyi entropy ($\alpha > 0$ and $\alpha \neq 1$) $H_\alpha(X)$ is given by:
\begin{equation}
    H_\alpha(X) = \frac{1}{1 - \alpha} \log \left( \int_X p^\alpha(x) \, dx \right),
\end{equation}
where $X$ is a continuous random variable with the probability density function (PDF) $p(x)$, and $\alpha$ is a positive constant.  
%and $\alpha > 0 \wedge \alpha \neq 1$. 
Rényi entropy extends the well-known Shannon entropy which is obtained when the parameter $\alpha$ approaches $1$~\citep{renyi1965foundations}.
%As $\alpha$ approaches $1$, Rényi entropy converges to the well-known Shannon entropy.
%$$
%H(X) = - \int_X p(x) \log p(x) \, dx
%$$
%The choice of $\alpha$ depends on the application. If $\alpha < 2$ or close to 1 is useful for estimating distribution tails or multiple modes. Otherwise, if $\alpha > 2$ highlights the average behavior, focusing on the main mode.

Calculating Rényi entropy requires knowing the PDF, which limits its application in data-driven context. To overcome this, we employ a matrix-based $\alpha$-order Rényi entropy calculation \citep{giraldo_2014_measures} %is proposed . This method resembles quantum Rényi entropy and that 
which computes Rényi's $\alpha$-order entropy using the eigenspectrum of a normalized Hermitian matrix, derived by projecting data into a Reproducing Kernel Hilbert Space (RKHS) \citep{gong2022computationally}:
\begin{equation}
S_\alpha(G) = \frac{1}{1 - \alpha} \log_2 \left( \text{tr}(G^\alpha) \right) = \frac{1}{1 - \alpha} \log_2 \left( \sum_{i=1}^n \lambda_i^\alpha(G) \right),    
\label{eq:Renyi_matrix_based}
\end{equation}
where $G$ is a normalized kernel matrix and $\lambda_i(G)$ are the eigenvalues of $G$. Specifically, each element of $G$ is $G_{ij} = \frac{1}{n} \frac{K_{ij}}{\sqrt{K_{ii} K_{jj}}}$, where $K$ is a Gram matrix with $K_{ij} = \varphi(x_i, x_j)$, and $\varphi$ is a real valued positive kernel that is infinitely divisible, and $x_i$ and $x_j$ are features of data samples extracted through filter $(1, 1024)$. %, and $\lambda_i(G)$ are the eigenvalues of $G$. Gram matrix $K$ obtained from 

\mv{How is G derived or formed from the data? If the data is the feature, how to form G?? Are $x_i, x_j$ data, are they elements of a feature matrix? What is n ??}

%For multiple variables, given a collection of $n$ samples $\{s_i = (x_i^1,x_i^2,\ldots,x_i^L)_{i=1}^{n}\}$, each sample contains $L$ ($L\ge2$) measurements $x^1 \in \mathcal{X}^1,x^2 \in \mathcal{X}^2,\ldots,x^L \in \mathcal{X}^L$ obtained from the same realization, and the positive definite kernels $\varphi_1$: $\mathcal{X}^1 \times \mathcal{X}^1 \mapsto \mathbb{R}, \varphi_2: \mathcal{X}^2 \times \mathcal{X}^2 \mapsto \mathbb{R}, \ldots, \varphi_L: \mathcal{X}^L \times \mathcal{X}^L \mapsto \mathbb{R}$. The matrix-based Rényi $\alpha$-order joint entropy for $L$ variables is \citep{yu_2019_multivariate}:
%\begin{equation} \label{eq:mi_multivar}
%S_\alpha(G_1, G_2, \ldots, G_L) = S_\alpha \left( \frac{G_1 \circ G_2 \circ \cdots \circ G_L}{\text{tr}(G_1 \circ G_2 \circ \cdots \circ G_L)} \right),
%\end{equation}
%where $(G^1)_{ij} = \varphi_1(x_i^1, x_j^1), (G^2)_{ij} = \varphi_2(x_i^1, x_j^1), \ldots, (G^L)_{ij} = \varphi_1(x_i^L, x_j^L)$, and $\circ$ denotes the Hadamard product.

For multiple variables, the matrix-based Rényi's $\alpha$-order  joint entropy of $L$ variables is computed as \citep{yu_2019_multivariate}
\begin{equation} \label{eq:mi_multivar}
S_\alpha(G_1, G_2, \ldots, G_L) = S_\alpha \left( \frac{G_1 \circ G_2 \circ \cdots \circ G_L}{\text{tr}(G_1 \circ G_2 \circ \cdots \circ G_L)} \right),
\end{equation}
where $(G^k)_{ij} = \varphi_k(x_i^k, x_j^k)$, with $k \in \{1,...,L\}$ denotes the normalized kernel matrix of the k$^{th}$ variable, and $\varphi_k$: $\mathcal{X}^k \times \mathcal{X}^k \mapsto \mathbb{R}$ is the k$^{th}$ positive definite kernel, and $\circ$ denotes the Hadamard product.

Using Rényi entropy, the matrix-based Rényi's $\alpha$-order mutual information $I_\alpha(\cdot; \cdot)$ is computed as
\begin{equation}
    I_\alpha(G; G_1, \ldots, G_L) = S_\alpha(G) + S_\alpha(G_1, \ldots, G_L) - S_\alpha(G_1, \ldots, G_L, G)
\end{equation}

% \[
% T_\alpha(G_1, \ldots, G_L) = \left( \sum_{i=1}^L S_\alpha(G_i) \right) - S_\alpha(G_1, \ldots, G_L).
% \]

% These matrix-based entropy measures are invariant to the order of the kernel matrices $G_1, \ldots, G_L$ and do not depend on the specific dimensions of the variables $x_1, \ldots, x_L$. This makes them suitable for high-dimensional data, whether discrete or continuous.

%\mv{Need a section for CMI definition and how to compute CMI (using Reyni).}
%\\
%\\
\textbf{Conditional Mutual Information Computation using Rényi Entropy:} Conditional mutual information (CMI) quantifies the amount of information shared between two random variables, $X$ and $Y$, given the knowledge of a third variable $Z$. Typically, it is expressed using Shannon entropy as
\begin{equation}
    I(X;Y|Z) = H(X,Z) + H(Y,Z) - H(X,Y,Z) - H(Z)
\end{equation}
Using Rényi entropy, CMI can be generalized as the matrix-based Rényi $\alpha$-order CMI:
\begin{equation}\label{eq:cmi_matrix}
    I_\alpha(G_X;G_Y|G_Z) = S_\alpha(G_X, G_Z) + S_\alpha(G_Y, G_Z) - S_\alpha(G_X, G_Y, G_Z) - S_\alpha(G_Z),
\end{equation}
where $G_X, G_Y, G_Z$ are the normalized kernel matrices defined on the data samples of the variables $X$, $Y$, and $Z$, respectively.


